Glottal source estimation robustness: A comparison of sensitivity of voice source estimation techniques

This paper addresses the problem of estimating the voice source directly from speech waveforms. A novel principle based on Anticausality Dominated Regions (ACDR) is used to estimate the glottal open phase. This technique is compared to two other state-of-the-art well-known methods, namely the Zeros of the Z-Transform (ZZT) and the Iterative Adaptive Inverse Filtering (IAIF) algorithms. Decomposition quality is assessed on synthetic signals through two objective measures: the spectral distortion and a glottal formant determination rate. Technique robustness is tested by analyzing the influence of noise and Glottal Closure Instant (GCI) location errors. Besides impacts of the fundamental frequency and the first formant on the performance are evaluated. Our proposed approach shows significant improvement in robustness, which could be of a great interest when decomposing real speech.

==> abstract.tex <==
\fontsize{9}{11}\selectfont This paper addresses the problem of estimating the voice source directly from speech waveforms.
A novel principle based on Anticausality Dominated Regions (ACDR) is used to estimate the glottal open phase. This technique is compared
to two other state-of-the-art well-known methods, namely the Zeros of the Z-Transform (ZZT) and the Iterative Adaptive Inverse Filtering (IAIF) algorithms. Decomposition quality is assessed on synthetic signals through two objective measures: the spectral distortion and a glottal formant determination rate. Technique robustness is tested by analyzing the influence of noise and Glottal Closure Instant (GCI) location errors. Besides impacts of the fundamental frequency and the first formant on the performance are evaluated. Our proposed approach shows significant improvement in robustness, which could be of a great interest when decomposing real speech.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Thomas Drugman, Thomas Dubuisson, Alexis Moinet, Nicolas D'Alessandro, Thierry Dutoit\\
  \fontsize{9}{11}\selectfont
  \textit{TCTS Lab, Facult\'e Polytechnique de Mons, 31 Boulevard Dolez, 7000 Mons, Belgium}\\
  \fontsize{9}{11}\selectfont
  \textit{firstname.lastname@fpms.ac.be}\\[12pt]
}
%\author{{\textmd {\textbf }}\\
%  \fontsize{11}{13}\selectfont
%  \\
%  \fontsize{9}{11}\selectfont
%  \textit{}\\
%  \fontsize{9}{11}\selectfont
%  \textit{}\\[12pt]
%}

==> keywords.tex <==
\fontsize{9}{11}\selectfont Speech Processing, Speech Analysis, Voice Source, Glottal Formant


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{Glottal source estimation robustness}\\
% The Subtitle should have initial letters capitalized
\fontsize{13}{15}\selectfont \textit{A comparison of sensitivity of voice source estimation techniques}
}

